Reconstruct before Query: Continual Missing Modality Learning with Decomposed Prompt Collaboration

Pre-trained large multi-modal models (LMMs) exploit fine-tuning to adapt diverse user applications. Nevertheless, fine-tuning may face challenges due to deactivated sensors (e.g., cameras turned off for privacy or technical issues), yielding modality-incomplete data and leading to inconsistency in training data and the data for inference. Additionally, continuous training leads to catastrophic forgetting, diluting the knowledge in pre-trained LMMs. To overcome these challenges, we introduce a novel task, Continual Missing Modality Learning (CMML), to investigate how models can generalize when data of certain modalities is missing during continual fine-tuning. Our preliminary benchmarks reveal that existing methods suffer from a significant performance drop in CMML, even with the aid of advanced continual learning techniques. Therefore, we devise a framework termed Reconstruct before Query (RebQ). It decomposes prompts into modality-specific ones and breaks them into components stored in pools accessible via a key-query mechanism, which facilitates ParameterEfficient Fine-Tuning and enhances knowledge transferability for subsequent tasks. Meanwhile, our RebQ leverages extensive multi-modal knowledge from pre-trained LMMs to reconstruct the data of missing modality. Comprehensive experiments demonstrate that RebQ effectively reconstructs the missing modality information and retains pre-trained knowledge. Specifically, compared with the baseline, RebQ improves average precision from 20.00 to 50.92 and decreases average forgetting from 75.95 to 8.56. Code and datasets are available on https://github.com/Tree-Shu-Zhao/RebQ.pytorch

==> src/tab/tab_prompt_generation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t] 
    \caption{Comparison of different prompt pool generation methods.}
    \label{tab:prompt-generator}
    \begin{center}
    \begin{tabular}{@{}lrr@{}}
    \toprule
    Method & AP~($\uparrow$) & FG~($\downarrow$) \\ \midrule
    {\shortmethod} & \textbf{59.92} & 8.56 \\ \midrule
    L2P~\cite{DBLP:conf/cvpr/0002ZL0SRSPDP22} & 27.33 & \textbf{3.53} \\
    DualPrompt~\cite{DBLP:conf/eccv/0002ZESZLRSPDP22} & 45.29 & 6.55 \\ 
    
    \bottomrule
    \end{tabular}
    \end{center}
\end{table}
